To Pool or Not To Pool: Analyzing the Regularizing Effects of Group-Fair Training on Shared Models

In fair machine learning, one source of performance disparities between groups is over-fitting to groups with relatively few training samples. We derive group-specific bounds on the generalization error of welfare-centric fair machine learning that benefit from the larger sample size of the majority group. We do this by considering group-specific Rademacher averages over a restricted hypothesis class, which contains the family of models likely to perform well with respect to a fair learning objective (e.g., a power-mean). Our simulations demonstrate these bounds improve over a naive method, as expected by theory, with particularly significant improvement for smaller group sizes.

==> cyrusnotes_obsolete.tex <==
Suppose also some \emph{reference function} $h \in \HC$ such that
\begin{equation}
\label{eq:ref-eta}
\Malfare_{p} \left( i \mapsto \Risk(\loss \circ h, \ProbDist_{i}); \wv \right) \leq \eta
\end{equation}
for some $\eta \in \RNN$.
Note that $\eta$ can be probabilistically bounded from a small amount data, as multiple comparisons and overfitting do not need to be considered to estimate the malfare of a single hypothesis $h$.
With an appropriate union-bound based setup, this data can be shared with the learning process, though handling the dependence is slightly tricky.

This quantity is crucial, because it allows us to constrain our learning process to the subset of $\HC$ that will improve malfare, which is less likely to overfit than learning over all of $\HC$.
Furthermore, by the monotonicity axiom of malfare functions (which holds for the power-mean family), we can upper bound the (empirical) malfare of any hypothesis $h$ by examining only subsets of groups.
In other words, where $\lv^{\downarrow}_{i}$ is some lower-bound on group $i$ empirical risk (e.g., $0$), it holds that
\begin{equation}
\Malfare_{p}\left( i \mapsto \begin{cases} i \in \mathcal{I} & \ERisk(\loss \circ h, (\bm{x}_{i},\bm{y}_{i})) \\ i \not \in \mathcal{I} & \lv^{\downarrow}_{i} \end{cases}; \wv \right) \leq \Malfare_{p}\left( i \mapsto \ERisk(\loss \circ h, (\bm{x}_{i},\bm{y}_{i})); \wv \right) \enspace.
\end{equation}
This lets us restrict the class of functions $\HC$ that we must consider for group $i$ while only using data or knowledge from the remaining groups.
%
To this end, we define the \emph{restricted hypothesis class} for group $i$ as
\begin{equation}
\label{eq:restriction}
\HC^{(0)}_{i} \doteq \left\{ h \in \HC \, \middle| \, \Malfare \left( j \mapsto 0 \vee \1_{j \neq i } \left( \underbrace{\EExpect_{\bm{x}_{j}, \bm{y}_{j}} [\loss \circ h]}_{\textsc{Empirical Risk}} - \underbrace{\Bigl(2\ERade_{\bm{m}_{j}} \bigl(\loss \circ \HC, (\bm{x}_{j}, \bm{y}_{j}) \bigr) + \varepsilon \Bigr)}_{\textsc{Generalization Error Bound}}  \right) ; \wv \right)  \leq \eta \right\} \enspace.
 \end{equation}
If $\loss \circ \HC$ is convex (in some parameterization $\Theta$ of $\HC$), then the set $\HC^{(0)}_{i}$ is also convex.
Furthermore, if $\loss \circ \HC$ is strongly convex, then it is straightforward to bound the diameter of $\HC^{(0)}_{i}$, which is significant for many generalization bounds.
Similarly, $\HC^{(0)}_{i}$ can be bounded by the intersection of multiple ellipsoids in this case.


In other words, ideally we would have some
\begin{equation}
\label{eq:restriction:ideal}
\HC^{(0)*} \doteq \left\{ h \in \HC \, \middle| \, \Malfare \left( j \mapsto \underbrace{\Expect_{\ProbDist_{i}} [\loss \circ h]}_{\textsc{True Risk}} ; \wv \right)  \leq \eta \right\} \enspace.
 \end{equation}
However, this depends on true risk values for all groups, so we drop group $i$ and lower-bound the remaining group risks, and it thus holds (w.h.p.) that $\HC^{(0)*} \subseteq \HC^{(0)}_{i}$.


%TODO erisk notation

It is illustrative to consider two special cases: if the malfare operator is utilitarian, i.e., $\Malfare_{1}(\cdot; \wv)$, then the restriction operator considers a weighted sum of risk values and Rademacher averages (and some additional statistical error $\varepsilon$) for all other groups, i.e,
\begin{equation}
\label{eq:restriction-util}
\HC^{(0)}_{i} \doteq \left\{ h \in \HC \, \middle| \, \sum_{ \substack{ j=1 \\ j \neq i} }^{\NGroups} \wv_{j} \left( 0 \vee \left( \underbrace{\EExpect_{\bm{x}_{j}, \bm{y}_{j}} [\loss \circ h]}_{\textsc{Empirical Risk}} -  \underbrace{\Bigl( 2\ERade_{\bm{m}_{j}} \bigl(\loss \circ \HC, (\bm{x}_{j}, \bm{y}_{j}) \bigr) + \varepsilon \Bigr)}_{\textsc{Generalization Error}} \right) \right) \leq \eta \right\} \enspace,
\end{equation}
and if the malfare operator is egalitarian, it then can be expressed as the intersection of classes, i.e.,
\begin{equation}
\label{eq:restriction-egal}
\HC^{(0)}_{i} \doteq
    \bigcap_{ \substack{ j=1 \\ j \neq i} }^{\NGroups}
    \left\{ h \in \HC \, \middle| \, %\forall i \in 1, \dots, \NGroups: \ 
    %\left(
    \underbrace{\EExpect_{\bm{x}_{j}, \bm{y}_{j}} [\loss \circ h]}_{\textsc{Empirical Risk}} - \underbrace{ \Bigl( 2\ERade_{\bm{m}_{j}} \bigl(\loss \circ \HC, (\bm{x}_{j}, \bm{y}_{j}) \bigr) + \varepsilon \Bigr) }_{\textsc{Generalization Error}}
    %\right)
    \leq \eta \right\} \enspace.
\end{equation}
Similar analysis can be performed for arbitrary power-mean welfare functions, though the resulting classes may be less intuitive for interpretable.

We now ask the question, how much does a model trained to optimize the malfare objective perform on each group?
Practically speaking, we want to know whether this joint training procedure can produce better, or at least statistically more stable, outcomes for minority groups, for whom a dearth of data makes learning with statistical confidence and generalizability challenging.
In particular, it holds that the empirically-optimal $\hat{h}$ obeys (w.h.p.)
\begin{equation}
\label{eq:group-bounds}
\forall i: \ \abs{ \Risk(\hat{h}, \ProbDist_{i}) - \ERisk(\hat{h}, \ProbDist_{i}) } \leq 2\ERade_{\bm{m}_{i}} \bigl(\loss \circ \HC^{(0)}_{i}, (\bm{x}_{i}, \bm{y}_{i}) \bigr) + \varepsilon \enspace,
\end{equation}
which improves the na\"ive bound (attainable without joint training) of
\begin{equation}
\label{eq:group-bounds-naive}
\forall i: \ \abs{ \Risk(\hat{h}, \ProbDist_{i}) - \ERisk(\hat{h}, \ProbDist_{i}) } \leq 2\ERade_{\bm{m}_{i}} \bigl(\loss \circ \HC, (\bm{x}_{i}, \bm{y}_{i}) \bigr) + \varepsilon \enspace.
\end{equation}

%TODO: abs consistency.


TODO E hat D subscripts???

TODO: Furthermore [malfare conclusion?]

Now, observe that the empirically malfare optimal solution $\hat{h}$ will (\whp) be a member of the intersection of each groups restricted class, i.e.,
\[
\hat{h} \doteq \argmin_{h \in \HC} \Malfare \left( i \mapsto \ERisk(\hat{h}, \ProbDist_{i}); \wv \right) \in \bigcap_{i=1}^{\NGroups} \HC^{(0)}_{i} \enspace,
\]
since violating any group's restricted class would imply a final malfare value $\geq \eta$ (\whp).
Furthermore, we can bound the true malfare (\whp) of $\hat{h}$ as the malfare of per-group risk upper bounds, i.e., it holds that
\begin{align*}
& \Malfare \! \left( i \mapsto \Risk(\hat{h}, \ProbDist_{i}); \wv \right) \! \\
&\leq \Malfare \left( i \mapsto \ERisk(\hat{h}, \ProbDist_{i}) + 2\ERade_{\bm{m}_{i}} \bigl(\loss \circ \HC^{(0)}_{i}, (\bm{x}_{i}, \bm{y}_{i}) \bigr) + \varepsilon; \wv \right) & \textsc{\eqref{eq:group-bounds}, Monotonicity of $\Malfare(\cdot; \wv)$} \\
&\leq \Malfare \! \left( i \mapsto \ERisk(\hat{h}, \ProbDist_{i}) ; \wv \right) + 2 \Malfare \! \left( i \mapsto \ERade_{\bm{m}_{i}} \bigl(\loss \circ \HC^{(0)}_{i}, (\bm{x}_{i}, \bm{y}_{i}) \bigr) ; \wv \right) + \varepsilon \!\!\enspace. \! & \textsc{Subadditivity of $\Mean_{p\geq 1}(\cdot; \wv)$} %{of $p \geq 1$ Power-Means} %\\
\end{align*}

Similarly, we may conclude that
\begin{equation}
\label{eq:malfare-opt}
\Malfare \! \left( i \mapsto \Risk(\hat{h}, \ProbDist_{i}); \wv \right) \! \leq \argmin_{h^{*} \in \HC} \Malfare \left( i \mapsto \Risk(h^{*}, \ProbDist_{i}); \wv \right) + 4 \Malfare \! \left( i \mapsto \ERade_{\bm{m}_{i}} \bigl(\loss \circ \HC^{(0)}_{i}, (\bm{x}_{i}, \bm{y}_{i}) \bigr) ; \wv \right) + 2\varepsilon \enspace.
\end{equation}

\medskip

[TODO: Under what conditions is this a good bound?]

[TODO: Contrast with multi-task learning bounds, which bound the sum of errors over tasks.]

%[TODO: Dependence DAG; each group's restricted class can use Rademacher averages of restricted classes of larger groups, if we get a DAG?]


\paragraph{Sources of Looseness}

One source of looseness is that Rademacher averages are taken separately for each group, whereas in the utilitarian case, they could be taken for the entire weighted loss objective all at once, though the strategy is difficult to generalize to arbitrary power-means.
Another source of looseness is that unconstrained Rademacher averages are used to construct the restricted hypothesis class $\HC^{(0)}_{i}$. This process can be repeated using the restricted class $\HC^{(0)}_{i}$ to construct $\HC^{(1)}_{i}$, and so on, iteratively, to converge to a smaller class $\HC^{(\infty)}_{i}$, though the analysis of this method is much more challenging, and computational hurdles must be overcome in the fixed point.

Ideally, we would be able to use data from group $j$ in its own restriction, i.e., take
\[
\HC^{(0)}_{*} \doteq \left\{ h \in \HC \, \middle| \, \Malfare \left( j \mapsto \EExpect_{\bm{x}_{j}, \bm{y}_{j}} [ \loss \circ h] + 2\ERade_{\bm{m}_{j}}(\loss \circ \HC, (\bm{x}_{j}, \bm{y}_{j}) )  + \varepsilon ; \wv \right)  \leq \eta \right\} \enspace,
\]
however this introduces a cyclic dependency of the class on the data, and greatly complicates the statistical analysis. However, the cost of omitting group $j$ is generally small, particularly if it is \emph{small} (i.e., has relatively low weight $\wv_{i}$) and has optimal risk comparable to the reference solution malfare.
Such an approach flirts with localization methods, which may be effective in some cases and are certainly of theoretical interest, however they add great analytic complexity overhead, and generally large constant factors to bounds.





==> old.tex <==

\subsection{Categories of relevant distributions to look at}

Recall the dimensions we are trying to understand the interactions between:

\begin{itemize}
\item Similarity of label distributions $P(Y|X,A)$
\item Similarity of feature distributions $P(X|A)$
\end{itemize}

\paragraph{Case 1: same label distributions, same feature distributions}

Sharing is caring. They're the same joint distribution. The end!



\paragraph{Case 2: same label distributions, different feature distributions}
As the "benefit of splitting" paper argues, if we had infinite data and knew the hypothesis class, knowing $P(Y|X,a) = P(Y|X,b)$ is sufficient to claim that \emph{sharing data always benefits both groups}. 

However, because of our sample size differences and our lack of assumptions about the hypothesis classes involved, we need stronger assumptions, particularly that $h*_a = h*_b$. If an improperly chosen hypothesis class is used, the model might approximate to the majority group well but generalize poorly to the part of the feature space where the minority group is. \todo{Can this example be explained with our framework or nah?}


The notion of model multiplicity (multiple possible $h*$s) also comes into play. The linear example in separate-variables shows a 2d linear case where only one variable's parameter matters for one group, and only the other variable's parameter matters for the other group. (Joint model can be expressed as sum of independent components) Only the jointly trained model $h*$ which learns both parameters fits both groups well, but each separately trained model only performs well on its own group and doesn't generalize to the rest of the feature space. Sharing does not hurt the groups but doesn't benefit them either. \todo{Implement, see what happens? Might not be interesting}


\paragraph{Case 3: different label distributions, same feature distributions}
This is the world of the ``discrepancy-overfitting" tradeoff that originally motivated our paper. (In the infinite-data setting, Benefit of Splitting paper proved that the benefit of splitting is exactly determined by the discrepancy between label distributions, but that is not our setting.) We want to run experiments where we can smoothly vary the difference in label distributions and the difference in sample sizes. (Recall: Groups with slightly different linear parameters and the resulting loss ellipses in simulation-examples; this regression problem is described in the following section.)


Experiments which capture this dynamic, which we've been focusing on, try to smoothly vary factors which change the \emph{threat of overfitting} (parameterized by sample size, hypothesis class and/or data generation process complexity, and noise) and the \emph{similarity of the label distributions} (parameterized by, well, model parameters, for one thing, but could be other things!).

What we would hope to see is that comparing the separate model generalization bound and (our original, tight) joint model generalization bound changing in ways we'd expect along these axes. That is: The higher the risk of overfitting for the minority group, the more beneficial joint training should be, and the tighter the joint model generalization bound.

Another interesting edge case explored in simulation: When $P(Y|X,a)=1-P(Y|X,b)$, we have two groups that are completely incompatible, and each group would be better off being treated separate, as the example in the intro describes. Still, the "cost" of sharing may still depend on how strong the signal is actually in the data (i.e. how far those probabilities are from 1/2 -- see decision trees in simulation examples). Interestingly(?) the joint model's groupwise generalization error's relationship with sample size may not be smooth (see: simple decision trees). \todo{Unsure if theory will be able to capture this}

\paragraph{Case 4: different label distributions, different feature distributions}

May want to run above experiment while also smoothly varying the difference between feature distributions in some sense.

(Todo: add a ``shared" variable to separate variable simulation get at this case? Label distributions and feature distributions are different but related.)






\paragraph{Realizable or Noisy Realizable Linear Regression}

We now consider a
%model
setting
in which no trade-offs need to be made across groups, and thus fair learning over all groups can be expected to perform even better than in the general case.
%Suppose the conditional distribution $Y | Z = i, X = x$ is constant across groups for all points $x$ and groups $i$, and
Suppose the conditional expectations $\Expect[Y | X = x]$ are linear in $X$ for all points $x$ and groups $i$.
Suppose also $X | Z = i$ is not constant across groups.

In this case, minority group predictions are only inaccurate if their $\vec{x}_{i}$ values fall significantly outside of the range of those encountered frequently in other groups (where frequently means sufficiently often so as to accurately approximate with respect to loss).
In the extreme, we can assume there exists some dimension $i$ such that the dimension $\vec{x}_{i}$ is $0$ or constant for all groups except group $j$, and the weights parameter $\vec{w}_{i}$ must then be learned using only group $i$ data.
In general, I think the property that would make any group difficult to predict is if the raw variance or sum of square values of some dimension $i$ is significantly greater than for any other group.

In any case, I suspect some notion of utilitarian training is an effective strategy, as even if each group is only useful to learn a subset of the weights variables, pooling data across groups helps to learn them all.
For example, if group one has data distribution $\langle 1, 0, \mathcal{N}(0, 1) \rangle$ and group 2 has $\langle 0, 1, \mathcal{N}(0, 1) \rangle$, then $\vec{w}_{1}$ can be learned from group $1$, $\vec{w}_{2}$ from group 2, and $\vec{w}_{3}$ from both.
Each group is also ill-conditioned on its own, and cannot distinguish between a constant linear offset and their constant $1$ dimension, but taken together they are well-conditioned.



==> rms.tex <==

\ccnote{RMS stuff:}

For the plots with the generalization bounds and the generalization error, averaging over multiple runs helps a lot, but the generalization error is still pretty unstable. Even after taking the absolute value, so at least it's non-zero, it can get very close to zero on some iterations and be far from zero on others.
Because of this “getting lucky” with near-0s phenomenon, I think we have a lot of “small outliers” contributing to the chaos.  I am thus also more interested in statistics that look like the maximum (over multiple runs) of generalization error than the average.

However, maxima have their own stability issues, so I’m proposing an RMS approach (i.e., plot the root mean squared generalization error, instead of the average).
One way to think about it is that the generalization error is already some kind of deviation, so the square root of the mean square generalization error actually makes sense on its own as a deviation metric (mean square error deviation).
Another way of thinking about that is that the root mean square is the 2 power mean, which is in some sense halfway between the average and the maximum.
The third way of thinking about it is that, because generalization error can be negative, we could take the square of generalization error and visualize that (instead of what we have now, which is kind of like a “mean absolute deviation”). However, we want the units and scale to match up with our generalization plots, so we just take the square root after averaging.
From this third perspective, I think it makes sense to compute the mean squared error, and also +- 1 standard deviation of square error, but then plot the square root of MSE and square root of MSE +- 1 stdev.

It's also worth noting that, since we are really looking at the large scale behavior of very small quantities, the log log plot is the right tool for the job, but it really magnifies any sort of weirdness around zero. This is part of why we need to average over multiple runs: the average of the logarithm has much much higher variance than the logarithm of the average. Looking at maximum or RMS statistics also helps here, anything that can shift the plot upwards reduces the logarithmic distance, and the RMS is no less than the average.

There are also other considerations at play: I haven't thought about it much, but median plus or minus quartiles may be more stable than mean plus minus standard deviation in this setting, it might be worth a look.

Finally, I worry that, ironically, removing the noise from the logistic regression labeling model might actually make this plot appear noisier, since an overall easier learning problem will have smaller risk values. It's probably too late to change that, but it might be worth thinking about if something is counterintuitive.

If all else fails: we can plot the generalization error until some sample size threshold, or just truncate the y-axis early, and explain that we did so because it essentially becomes noise after this point, and the main point of this plot is really to study the generalization bounds. With more space, I'd like to have a small-scale plot that has everything on natural axes, and a large scale plot that just has the generalization bounds. Maybe we could do that, but put the small-scale plot in the appendix instead?

